The Canonical Distortion Measure for Vector Quantization and Function Approximation

To measure the quality of a set of vector quantization points a means of measuring the distance between a random point and its quantization is required. Common metrics such as the {\em Hamming} and {\em Euclidean} metrics, while mathematically simple, are inappropriate for comparing natural signals such as speech or images. In this paper it is shown how an {\em environment} of functions on an input space $X$ induces a {\em canonical distortion measure} (CDM) on X. The depiction 'canonical" is justified because it is shown that optimizing the reconstruction error of X with respect to the CDM gives rise to optimal piecewise constant approximations of the functions in the environment. The CDM is calculated in closed form for several different function classes. An algorithm for training neural networks to implement the CDM is presented along with some encouraging experimental results.

==> abstract.tex <==
\begin{abstract}
To measure the quality of a set of vector quantization points a means
of measuring the distance between a random point and its quantization 
is required. Common
metrics such as the {\em Hamming} and {\em Euclidean} metrics, while
mathematically simple, are inappropriate for comparing natural signals such as speech 
or images. In this paper it is shown how an {\em environment} of
functions 
on an input space $X$  
induces a {\em canonical distortion measure} (CDM) on X.
The depiction ``canonical'' is justified because it is shown 
that optimizing the reconstruction
error of X with respect to the CDM gives rise to optimal
piecewise constant approximations of the functions in the environment. The CDM
is calculated in closed form for several different function classes.
An algorithm for training neural networks to implement the CDM
is presented along with some encouraging experimental results.
\end{abstract}



